Parameterized algorithms for Eccentricity Shortest Path Problem

Given an undirected graph $G=(V,E)$ and an integer $\ell$, the Eccentricity Shortest Path (ESP) asks to find a shortest path $P$ such that for every vertex $v\in V(G)$, there is a vertex $w\in P$ such that $d_G(v,w)\leq \ell$, where $d_G(v,w)$ represents the distance between $v$ and $w$ in $G$. Dragan and Leitert [Theor. Comput. Sci. 2017] showed that the optimization version of this problem, which asks to find the minimum $\ell$ for the ESP problem, is NP-hard even on planar bipartite graphs with maximum degree 3. They also showed that ESP is W[2]-hard when parameterized by $\ell$. On the positive side, Ku\v cera and Such\'y [IWOCA 2021] showed that the problem exhibits fixed parameter tractable (FPT) behavior when parameterized by modular width, cluster vertex deletion set, maximum leaf number, or the combined parameters disjoint paths deletion set and $\ell$. It was asked as an open question in the above paper, if ESP is FPT parameterized by disjoint paths deletion set or feedback vertex set. We answer these questions partially and obtain the following results: - ESP is FPT when parameterized by disjoint paths deletion set, split vertex deletion set or the combined parameters feedback vertex set and eccentricity of the graph. - We design a $(1+\epsilon)$-factor FPT approximation algorithm when parameterized by the feedback vertex set number. - ESP is W[2]-hard when parameterized by the chordal vertex deletion set.

==> conclusion.tex <==
\section{Conclusion}
In this paper, we studied \textsc{Minimum Eccentricity Shortest Path} problem from the viewpoint of parameterized complexity. We show that the problem is FPT when parameterized by feedback vertex set and eccentricity of the graph. 
%by giving an MSO$_2$ formula. We also give an explicit FPT algorithm for the problem parameterized by feedback vertex set and the eccentricity of the graph. 
However, we could not adapt our algorithm to design an FPT algorithm with feedback vertex set alone. We design a $(1+\epsilon)$-factor approximation algorithm when parameterized by the feedback vertex set number. 
We also give FPT algorithms parameterized by disjoint paths deletion set or split vertex deletion set. We complement this by showing that the problem is {\sf W}[2]-hard when parameterized by chordal vertex deletion set.  

We conclude with the following list of open questions:
\begin{itemize}
    \item What is the parameterized complexity of the problem when parameterized by feedback vertex set, tree-width, clique-width, tree-width or interval vertex deletion set. 
\end{itemize}
%\textsc{Eccentricity Shortest Path}

==> fvs-mso.tex <==
\subsection{MSO$_{2}$ Formulation of \amesp}\label{sec:mso}
%Given a forest $F$, a set $B\subseteq V(F)$, 
%an integer $\ell$, and a family $\cF=\{\cF_1,\cF_2,\dots ,\cF_t\}$ of $t$ disjoint families of feasible paths.
In this section, we show that the \amesp problem can be expressed as a MSO$_2$ formula. Given a forest $F$, a set $B\subseteq V(F)$, 
an integer $\ell$, and a family $\cF=\{\cF_1,\cF_2,\dots ,\cF_t\}$ of $t$ disjoint families of feasible paths, we define a distance matrix that has 0-1 entries based on whether the distance between a vertex in $B$ and a path $P$ is at most $\ell$ or not, formally as follows:

\begin{equation*}
    Dist(v,p_i) =
    \begin{cases}
      1 & \text{if }  d_G(v, p_i)\leq \ell,\\
       0 & \text{otherwise. }\\ 
       %dist_G(v, p_i)> \ell\\
    \end{cases}
\end{equation*}


We express the \amesp problem  as a MSO$_2$ formula $\phi_t$ in the following way: 
$$\phi_{t}=\exists_{p_1\in \mathcal{F}_1 , p_2\in \mathcal{F}_2, \dots , p_t\in \mathcal{F}_t}  Eccentric(p_1, p_2, \dots, p_t,B)$$ 
where $Eccentric(\dots)$ is a subformula that expresses every vertex in $B$ is  at a distance of at most $\ell$ from some path $p_i$, where 
$i\in \{1, 2, \dots, t\}$. We express $Eccentric(\dots)$ as follows: 
%there exists a path $p_i$ chosen from $\mathcal{F}_i$ for each $i\in \{1, 2, \dots, t\}$, such that each vertex in $B$ is
$$Eccentric(p_1, p_2, \dots, p_k, B)=\bigwedge\limits_{\forall b\in B  } \Bigl(Dist(b, p_1)\lor Dist(b, p_2)  \lor \dots \lor Dist(b, p_k)\Bigr).$$ %and 
%%where $Dist(b, p_i)$ represents a boolean value whose value is 1 is the distance between $b$ and $p_i$ is at most $\ell$ and 0 otherwise. Formally, 



%that every vertex in $B$ is at a distance of at most $\ell$ from some path $p_i\in $, where $i\in \{1, 2, \dots, t\}$, chosen from $\mathcal{F}_i$. 
%given the path $p_i$ is chosen from $\mathcal{B}_i$, for each $i\in [t]$, each vertex in 


%$$\exists\limits_{p_1, p_2,\dots , p_t(p_1\in \mathcal{F}_1 \land p_2\in \mathcal{F}_2 \land \dots \land p_t\in \mathcal{F}_t)} \land satisfy()$$

%$Eccentricity(p_1, p_2, \dots, p_k, B)$ indicates that the paths chosen  

\begin{theorem}\label{thm:col-path-mso}
\amesp is FPT when parameterized by $t$. 
\end{theorem}
\begin{proof}
The \amesp problem is expressible in MSO$_2$ as shown above. Using Courcelle's theorem \cite{COURCELLE199012} we get that \amesp is FPT when parameterized by tree-width and $t$. Since the input graph is a forest, the tree-width of the graph is one. Hence we get that \amesp is FPT when parameterized by $t$ alone. 
\end{proof}


%Using Observation \ref{lem:skelnum}, Lemma \ref{lem:mespfvscorr} and Lemma \ref{lem:disjointfvscorr}, we get that \mespfvs is solvable in FPT time. 

==> fvsdp-sri.tex <==
\subsection{Proof of Theorem \ref{thm:annotated}: Algorithm for \annotatedmesp}\label{sec:annotated}

In this section, we design a dynamic programming based FPT algorithm for the \amesp problem. Notice that input to \amesp is a forest, although we can independently work with each connected component of forest. Therefore, from now onwards we assume that the input is restricted to a tree.  
%In particular,  we prove \cref{thm:annotated}. 
Consider an instance $(T,B,\ell,\cF =\{\cF_1,\cF_2,\dots \cF_t\})$ of \amesp problem. Where $T$ is a tree, $B\subseteq V(T)$, $\ell\in \mathbb{N}$, and $\cF$ satisfying the following: \textbf{(a)} Each $\cF_i$, $i\in [t]$ is a set of paths in $T$, 
\textbf{(b)} $V(\cF_i)\cap V(\cF_j)=\emptyset$, for all $i,j\in [t], i\neq j$, and 
\textbf{(c)} Let $u, v\in V(T)$ be two vertices such that $v$ is the parent of $u$. If $F(u)\neq 0$ and $F(v)\neq 0$, then $F(u)=F(v)$. 
    

\begin{comment}
\begin{itemize}
    \item[1.] Each $\cF_i$, $i\in [t]$ is a set of paths in $T$, 
    \item[2.] $V(\cF_i)\cap V(\cF_j)=\emptyset$, for all $i,j\in [t], i\neq j$, and 
    \item[3.] Let $u, v\in V(T)$ be two vertices such that $v$ is the parent of $u$. If $F(u)\neq 0$ and $F(v)\neq 0$, then $F(u)=F(v)$. 
    
 
\end{itemize}

\end{comment}



The aim is to find a set $\cal P$ of $t$ paths such that for each $\cF_i$, $i\in [t]$, $|\mathcal{P}\cap \cF_i|=1$ and for every vertex $v\in B$, there exists a path $P\in {\cal P}$ and a vertex $u\in V(P)$, such that $d_T(u,v)\leq \ell$. 
Notice that an instance of \amesp is generated from an instance of \dmesp. The latter ensures that the paths in $\mathcal {F}$ are such that if there are 
two adjacent vertices $u$ and $v$ for which $F(u)\neq 0$ and $F(v)\neq 0$, 
then $F(u)=F(v)$. Otherwise, there is a shortest path $m_{F(v)} - \dots - v - u - \dots - m_{F(u)+1}$, contradicting to the fact that the \dmesp is an yes instance. Hence the existence of \textbf{(c)} is justified. This will help in simplifying many of the cases in the dynamic programming algorithm. 

%The existence of (3) ensures that the paths considered in $\mathcal{F}$ are from \dmesp and 



% (3) If there exists two paths $P_1,P_2\in \cF_i$, $i\in [t]$, with endpoints $u_1,v_1$ and $u_2,v_2$, respectively, such that $V(P_1)\cap V(P_2)\neq \emptyset$, then there exists a vertex $v\in V(P_1)\cap V(P_2)$ such that $P_1$ and $P_2$ are paths that passes through $v$ and one of the following holds: 
%(i) Their endpoints are distinct, i.e., $u_1\neq u_2, u_1\neq v_2, v_1\neq u_2, v_1\neq v_2$ and 
%
%$V(P_1)\cap V(P_2)= \{v\}$.
%
%(ii) One of the endpoint is equal, for example $u_1=u_2$ and $v_1\neq v_2$ (other cases are analogous), in this case let $P'$ be the $v$ to $u_1$ subpath in $T$, then $V(P_1)\cap V(P_2)= V(P')$. 





%We design a dynamic programming algorithm. Intuition..



\noindent\textbf{Description of the Algorithm:} %First we give the description of our algorithm. 
The algorithm starts by arbitrarily rooting tree $T$ at a root $r\in V(T)$. 
%From now onwards, we assume that $T$ is rooted at $r$. 
In the following, we state some notations, which will be used in the algorithm. For a vertex $v\in V(T)$, we denote the number of children of $v$ in $T$ by $deg(v)$. By $T_v$, we denote the subtree of $T$ rooted at $v$. By $\sch^v_i$, we denote $i$th child of $v$. 
For a vertex $v\in T$, and  $0 \leq i\leq deg(v)$, we define $T_{v,i}$ as the subtree of $T$ containing vertex $v$ and subtrees rooted at its first $i$ children (in order of index). Also,  $T_{\sch^v_j}$ is the 
subtree of $T$ containing vertex $v$ and subtrees rooted at its  $i$th child. 


Recall that every vertex $v\in V(T)$ can be contained in at most one $\cF_i$, $i\in[t]$. For each vertex $v\in V(T)$, we assign a value $F(v)\in [0,t]$ to $v$ as follows: $F(v)=i$, if $v\in V(\cF_i)$, and 
$0$ otherwise (when no path in any $\cF_i, i\in [t]$ contain $v$). 
Recall that   a path $P$ {\em covers} a vertex $v$ if there exists a vertex $u\in V(P)$ such that $d_{G}(v,u)\leq \ell$. For a vertex $v\in V(T)$, dynamic programming algorithm considers subproblems for each child of $v$. We process its children from left to right (in index ordering) and at $i$th child, we consider subtree $T_{v,i}$. Before we define an entry in the table, we give the definition of the variables used for an entry. 

  
 Consider $v\in V(T)$ and $i\in [deg(v)]$. To compute partial solution at subtree $T_{v,i}$, we have to distinguish whether $v$ is contained in a path in the solution. If it is contained in a path in the solution, then we also guess where  the endpoints of the path are. For this purpose, we define a variable $\stype$ which can take a value from the set $\{1, 2, \dots, 11\}$, where each value represents a different case defined as follows: 
 \begin{itemize}
     \item\textbf{tp=1:} Paths containing $v$ are not in the solution. 
     \item\textbf{tp=2:} The vertex $v$ itself is a path that is contained in the solution. 
     
     %For the remaining cases we have that a path containing $v$ is in the solution with the following added conditions: 
     
     %For $\stype\in \{3,4,5,6\}$, cases {\bf (3),(4),(5)} and {\bf (6)} we have condition that path also contains parent of $v$: with the following added conditions:
    \item\textbf{tp} \boldmath{$\in \{3, 4, 5, 6\}$}: For all these cases, we have the parent of $v$ in the solution, in addition to satisfying their respective properties.   
    \begin{itemize}
        \item\textbf{tp=3:} One of its endpoints is $v$ itself. 
        \item\textbf{tp=4:} One of its endpoints is in $T_{v,i-1}$ ($\neq v$). 
        \item\textbf{tp=5:} One of its endpoints is in $T_{\sch^v_i}$ ($\neq v$). 
        \item\textbf{tp=6:} One of its endpoints is in $T_{\sch^v_j}$ for some $j>i$ ($\neq v$). 
    \end{itemize}
    \item\textbf{tp=7:} Both of its endpoints are in $T_{v,i-1}$ (at least one endpoint is not equal to $v$).
    \item\textbf{tp=8:} One of its endpoints is in $T_{v,i-1}$, and the other 
    %other endpoint is 
    in $T_{\sch^v_i}$ ($\neq v$).  
    \item\textbf{tp=9:} One of its endpoints is in $T_{v,i-1}$, and the other 
    %endpoint is 
    in $T_{\sch^v_j}$ for some $j>i$ ($\neq v$). 
    \item\textbf{tp=10:} One of its endpoints is in $T_{\sch^v_i}$, and the 
    other 
    %endpoint is 
    in $T_{\sch^v_j}$ for some $j>i$ ($\neq v$). 
    \item\textbf{tp=11:}   One of its endpoints is in $T_{\sch^v_j}$ for some $j>i$, and 
    the other 
    %endpoint is 
    in $T_{\sch^v_{j'}}$ for some $j'>i$ ($\neq v$). 
  
%\item $\bf 10$ represents that a path containing $v$ is in the solution and both of its endpoints are in $T_{\sch^v_i}$ (at least one endpoint is not equal to $v$).
  
 

 \end{itemize}

%\end{itemize}


\begin{figure}[ht!]
	\centering
	\includegraphics[width=.8\textwidth]{5.pdf}
	\caption{.}
	\label{fig:dp}
\end{figure}


\begin{sloppypar}
We have a variable $(\ssign)\srem$. Here $\ssign$ represents sign of $\srem$, which can either be $+$ or $-$, 
and $(\ssign)\srem$ can take a value from the set $\{\sM\ell-1,\dots, \sM1, \sM0,\sP0,\sP1,\dots, \sP \ell\}$. The ``$-$'' sign represents that there are uncovered vertices in $V(T_{v,i})\cap B$ which needs to be covered in future, and ``$+$'' sign represents that all the vertices in $V(T_{v,i})\cap B$ are covered and the partial solution may cover more vertices outside $T_{v,i}$. 
The value $\sM\srem$ represents that the maximum distance of a vertex $u\in B$ from $v$ in subtree $T_{v,i}$ such that $u$ is not covered by the partial solution, 
is $\srem$. 
It means that vertices up to distance $\srem$ from $v$ in $V(T_{v,i})\cap B$ needs to be covered by some paths in future. We consider values only till $\ell-1$ distance, as it is a trivial observation that any vertex at distance at least $\ell$ from $v$ in $T_{v,i}$ cannot be covered by any path that is not in $T_{v,i}$. 
The value $\sP\srem$ represents that the minimum distance of a vertex $u$ in subtree $T_{v,i}$ ($u$ need not belong to $B$) 
such that distance from $u$ to $v$ is $\ell-\srem$ and $u$ is contained in a path in the solution. 
This implies that $v$ can cover vertices up to  distance $\srem$ in future. 
In the following definition, we state the entries in our dynamic programming routine.
%\textcolor{red}{such that there exists a vertex $u\in B$ in subtree $T_{v,i}$ such that distance from $u$ to $v$ is $\ell-\srem$ and $u$ is contained in a path in the solution. It means that vertices in $B$ which are at distance at most $\srem$ from $v$ (at most $\ell$ from $u$) in $T$ can be covered by a path containing $u$ in the solution. In the following definition, we state the entries in our dynamic programming routine. }
 
%We have a variable $\srem$, it can take a value from set $[-1,\ell-1]$ which represents maximum distance of a vertex $u$ from $v$ in subtree $T_{v,i}$ such that $u$ is not covered by the partial solution. It means that vertices up to distance $\srem$ from $v$ in $T_{v,i}$ needs to be covered by some paths in future. $-1$ represents that all the vertices in $T_{v,i}$ are covered. We consider only till $\ell-1$ distance, as it is a trivial observation that any vertex at distance at least $\ell$ from $v$ in $T_{v,i}$ cannot be covered by any path that is not in $T_{v,i}$.
%
%We have a variable $\sf ext$, it can take a value from the set $[0,\ell]$, it represents that (1) every vertex in $T_{v,i}$ is covered and (2) $\sf ext$ is the minimum value such that there exists a vertex $u$ in subtree $T_{v,i}$ such that distance from $u$ to $v$ is $\ell-\sext$ and $u$ contained in a path in the solution. It means that vertices at distance at most $\sf ext$ from $v$ ( at most $\ell$ from $u$) should be covered by a path contaning $u$ in the solution.


%We have a variable $\srem$, it can take a value from set $[-1,\ell-1]$ which represents distance from $v$ to a vertex $u$ in subtree $T_{v,i}$ such that $v$ is not covered by the partial solution. It means that vertices up to distance $\srem$ from $v$ in $T_{v,i}$ needs to be covered by some paths in future. $-1$ represents that all the vertices in $T_{v,i}$ are covered. We consider only till $\ell-1$ distance, as it is a trivial observation that any vertex at distance at least $\ell$ from $v$ in $T_{v,i}$ cannot be covered by any path that is not in $T_{v,i}$.
%
%We have a variable $\sf ext$, it can take a value from the set $[\ell]$, which represents $\ell$ minus minimum distance from $v$ to a vertex $u$ in subtree $T_{v,i}$ such that $u$ contained in a path in the solution. It means that vertices at distance at most $\sf ext$ from $v$ ( at most $\ell$ from $u$) should be covered by a path contaning $u$ in the solution.

% In the following definition, we state the entries in our dynamic programming routine.
% 
% \begin{definition} For each $v\in V(T)$, $d\in deg(v)$, $Y\subseteq [t]$,$\stype\in [12]$, ${\sf ext}\in [\ell], {\srem}\in [-1,\ell-1]$ we store an entry $c[v,d,Y,{\stype}, {\sf ext}, {\srem}]$ in our table which stores $\strue$ if and only if the following holds:

\begin{definition} \label{def:dp}
For each $v\in V(T)$, $d\in [deg(v)]$, $Y\subseteq [t]$, $\stype\in 
\{1, 2,\dots, 11\}, 
(\ssign)\srem \in\{\sM\ell-1,\dots, \sM1, \sM0,\sP0,\sP1,\dots, \sP \ell\}$, we create an entry $c[v,d,Y,{\stype},(\ssign) {\srem}]$ in our table which stores $\strue$ if and only if the following holds, otherwise $c[v,d,Y,{\stype}, (\ssign){\srem}]$ stores $\sfalse$:
 
 \noindent{\bf (1)} There exists a set $\cP_{v,d}$ of $|Y|$ paths such that for each $j\in Y$, $|\cP_{v,d}\cap \cF_j|=1$, if $F(v)\in Y$, then path in $\cP_{v,d}\cap \cF_{F(v)}$ should satisfy definition of $\stype$, and all paths in $\cP_{v,d}$ except maybe path containing $v$ should be contained in the subtree $T_{v,d}$. 
 
 \noindent{\bf (2)} If $\ssign$ is $-$, then there exists a vertex $u\in B$ at distance $\srem$  from $v$ in $T_{v,d}$ which is not covered by any paths in $\cP_{v,d}$ 
  but can be covered in future (is not at distance greater than $\ell$ from $v$). For every vertex $u\in B$ at distance at least ${\srem} +1$ from $v$ in subtree $T_{v,d}$ there exists a path in $\cP_{v,d}$ which covers $u$. 
 
\noindent {\bf (3)} If $\ssign$ is $+$, then for every 
vertex in $T_{v,d}\cap B$, there exists a path in $\cP_{v,d}$ which covers it. Further the minimum distance from $v$ to a vertex on a path in the solution path in $T_{v,d}$ is $\srem$. 
\end{definition}

%vertex $u\in B$ which is either in 
%$T_{v,d}$, or not in $T_{v,d}$ and at a distance at most ${\srem}$ from $v$ there exists a path in $\cP_{v,d}$ which covers $u$.  

\begin{comment}
\textcolor{red}{
\begin{observation}\label{obs:new-dp1}
Let $v\in V(T)$ and $w$ be a child of $v$ and 
the solution set $\mathcal{P}_{r, deg(r)}$ be the set of paths at root $r$, satisfying the rules of Definition \ref{def:dp}. If $v$ and $w$ belong to some paths $P$ in $\mathcal{P}_{r, deg(r)}$, then 
$F(v)=F(w)$. 
%$\mathcal{P}_{v,d}$ denote the set of paths in the solution satisfying Definition \ref{def:dp}. 
%If there exists a vertex $w\in N(v)$ such that $\mathcal{F}_{(F(w))}\in \mathcal{P}$, then $F(w)=F(v)$. 
%$f(w)\neq f(v)$. 
\end{observation}
\begin{proof}
%Suppose Since $v\in S$, we have that $F(v)\in [t]$. 
There are two cases depending on whether $v$ and $w$ belong to the same path or different paths in the solution. Let they belong to different paths. There exists a shortest path between endpoints (in $M$) 
in the path containing $v$ and the endpoints (in $M$) in the path of $w$. These are  not valid paths to be considered in the instance. The other case is that there is path containing $v$ and $w$ in the solution. Hence $F(v)=F(w)$. 
%Suppose $F(v)\neq F(w)$. That is there exists paths $P_v$ and $P_w$ passing through $v$ (and not $w$) and $w$ (and not $v$). 
%Let $P_v$ be the path in $\mathcal{}$the Then there exists a shortest path passing through the vertices of $M$ passing through $v$, $w$ and then to the vertices in $M$. 
\end{proof}}

\end{comment}

Observe that $(T,B,\ell,\cF=\{\cF_1,\cF_2,\dots,  \cF_t\})$ is a yes instance of \amesp if and only if there exists an entry $c[r,deg(r),\{1, 2, \dots, t\}, \stype^*,\sP\srem^*]$, $\stype^*\in \{1,2,7,8\}$ and  $\srem^* \in [0,\ell]$, which is set to $\strue$. Next, we give (recursive) formulas for the computation of entries in our dynamic programming table. %Their correctness can be found in \cref{sec:annotatedapp}~. 
Consider $v\in V(T),d\in [deg(v)],Y\subseteq [t],\stype\in [11],  (\ssign)\srem \in \{\sM\ell-1,\dots, \sM1, \sM0,\sP0,\sP1,\dots, \sP \ell\}$, 
we compute the entry $c[v,d,Y,{\stype}, (\ssign){\srem}]$ based on the following cases: 

\noindent{\bf Leaf vertex $v$:} 
%$v$ is a leaf vertex. 
Set $c[v,0,Y,{\stype}, (\ssign){\srem}]=\strue$, if one of the following holds: (a1) $\stype=1, (\ssign)\srem=\sM 0$, $Y=\emptyset$, or (a2) $\stype\in \{2,3\} , (\ssign)\srem=\sP\ell$, $Y=F(v)$. Otherwise set the entry to $\sfalse$. 
%Note that here $d=0$. 
Correctness follows trivially from the definition of entry. 

\noindent{\bf Non-leaf  vertex $v$:} 
%$v$ is not a leaf vertex. 
We consider the following cases depending on $\stype$ variable. 

\noindent {\bf Case  $\stype=1$:} We further consider following cases. \textbf{(1)} If $\ssign=-$, then set $c[v,d,Y,1,(-){\srem}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y$ such that one of the following holds: 
 (a1) $c[v,d-1,Y_1,1, (\ssign){\srem}_1]=\strue$, $(\ssign)\srem_1\in \{\sM\srem,\dots, \sP\srem-1\}$ and
 (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,\sM\srem-1]=\strue$, or,  
 (b1) $c[v,d-1,Y_1,1, \sM{\srem}]=\strue$, and
 (b2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,(\ssign)\srem_2]=\strue$, $(\ssign)\srem_2\in \{\sM\srem-1,\dots, \sP\srem\}$. 
 
 \textbf{(1.1)} If $\ssign=+$, then set $c[v,d,Y,1,(+)\ell -1]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y$ such that one of the following holds: (a1) $c[v,d-1,Y_1,1, (\ssign)\srem_1]=\strue$,   $(\ssign)\srem_1\in \{\sM\ell-2,\dots, \sP\ell-1\}$ and
 (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,\stype_2,\sP\ell]=\strue$, $\stype_2\in \{2,7,8\}$, or, 
  (b1) $c[v,d-1,Y_1,1, \sP\ell-1]=\strue$, 
  and
 (b2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,(\ssign)\srem_2]=\strue$, $(\ssign)\srem_2\in \{\sM\ell-2,\dots, \sP\ell-1\}$. 


\textbf{(1.2)} If $\ssign=+$ and $\srem<\ell-1$, then set $c[v,d,Y,1,(+){\srem}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y$ such that one of the following holds: (a1) $c[v,d-1,Y_1,1, (\ssign){\srem}_1]=\strue$,  $(\ssign)\srem_1\in \{\sM\srem,\dots, \sP\srem\}$ and
 (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,\sP\srem+1]=\strue$,  or
  (b1) $c[v,d-1,Y_1,1, \sP{\srem}]=\strue$,  and
 (b2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,(\ssign)\srem_2]=\strue$,  $(\ssign)\srem_2\in \{\sM\srem,\dots, \sP\srem+1\}$. 

%{\em Correctness}: Consider the case when (a1) and (a2) are true, then there exists a set of paths $\cP_1$ which set (a1) to true and there is a set of paths $\cP_2$ which set (a2) to true. We claim that $\cP=\cP_1\cup \cP_2$ is a solution to $c[v,d,Y,1,(-){\srem}]=\strue$. Observe that no path containing $v$ is in $\cP$, as $\stype_1,\stype_2\in \{1,2,7,8\}$. since $Y=Y_1\uplus Y_2$, we have that for each $i\in Y$, we have exactly one path in $\cP\cap \cF_i$. Next, observe that there exists a vertex $u\in B$ at distance $\srem$ from $v$ in $T_{\sch^v_d}$, which is not covered by paths in $\cP_1$. Also $(\ssign)\srem_1\in \{\sM\srem-1,\dots, \sP\srem\}$, it is not covered by  $\cP_2$, as any vertex in $\cP_2$ requires at least $\srem+1$ distance to reach $u$. Observe that every vertex at distance at least $\srem+1$ from $v$ in $T_{v,d}$ is covered by paths in $\cP$. Analogous arguments follows for the case when (b1) and (b2) are true.



 
 
 




%\bscomment{**}
%{\em Correctness}: Consider the case when (a1) and (a2) are true, then there exists a set of paths $\cP_1$ which set (a1) to true and there is a set of paths $\cP_2$ which set (a2) to true. We claim that $\cP=\cP_1\cup \cP_2$ is a solution to $c[v,d,Y,1,(+){\srem}]=\strue$. Observe that no path containing $v$ is in $\cP$, as $\stype_1,\stype_2\in \{1,2,7,8\}$. since $Y=Y_1\uplus Y_2$, we have that for each $i\in Y$, we have exactly one path in $\cP\cap \cF_i$. Next, observe that every vertex in $T_{\sch^v_d}$ is covered by $\cP_2$ and since  $(\ssign)\srem_1\in \{\sM\srem,\dots, \sP\srem+1\}$, every vertex in $T_{v,d-1}$ is covered either by $\cP_1$ or $\cP_2$. By (a2) we also satisfy $\sP\srem$, that is vertices at distance at most $\srem$ is covered by $\cP_2$. Analogous arguments follows for the case when (b1) and (b2) are true.

\noindent {\bf Case  $\stype=2$:} If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or $v$ is not a path in $\cF_{F(v)}$, then set $c[v,d,Y,2,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,2,(+)\ell]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1,2, \sP\ell]=\strue$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,(\ssign)\srem_2]=\strue$,  $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell-1\}$.


%{\em Correctness}: Suppose that (a1) and (a2) are true, then there exists a set of paths $\cP_1$ which set (a1) to true and there is a set of paths $\cP_2$ which set (a2) to true. We claim that $\cP=\cP_1\cup \cP_2 \cup \{v\}$ is a solution to $c[v,d,Y,2,(+)\ell]=\strue$. Observe that no path containing $v$ is in $\cP$, as $\stype_1,\stype_2\in \{1,2,7,8\}$. since $Y=Y_1\uplus Y_2\uplus \{F(v)\}$, we have that for each $i\in Y$, we have exactly one path in $\cP\cap \cF_i$. Next, observe that every vertex in $T_{\sch^v_d} \cup  T_{v,d-1}$ is covered by $\cP$ since  $(\ssign)\srem_1\in \{\sM\srem,\dots, \sP\srem+1\}$ and path containing $v$ is in $\cP$,  hence every vertex in $T_{v,d}$ is covered by $\cP$.

%\noindent {\bf Case 3} $\stype=3$ : If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, parent of $v$ and has one of its endpoint as $v$, then set $c[v,d,Y,3,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,3,(+)\ell]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},3, (+)\ell]=\strue$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,{\stype}_2,(\ssign)\srem_2]=\strue$,  $\stype_2\in \{1,2,7,8\}$, $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell\}$.
%% The correctness can be argued similar to Case 2.
%
%\noindent {\bf Case 4} $\stype=4$ : If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, parent of $v$ and has one of its endpoint in $T_{v,d-1}$ ( endpoint is not $v$), then set $c[v,d,Y,4,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,4,(+)\ell]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, $\stype\in \{3,4\}$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,{\stype}_2,(\ssign)\srem_2]=\strue$,  $\stype_2\in \{1,2,7,8\}$, $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell\}$.
% The correctness can be argued similar to Case 2.

 

\begin{sloppypar}
	\noindent {\bf Case $\stype=3$:}  If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, parent of $v$ and has one of its endpoint as $v$, then set $c[v,d,Y,3,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,3,(+)\ell]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},3, (+)\ell]=\strue$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,(\ssign)\srem_2]=\strue$, 
	$(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell-1\}$.
	% The correctness can be argued similar to Case 2.
	
	\noindent {\bf Case $\stype=4$:}  If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, parent of $v$ and has one of its endpoint in $T_{v,d-1}$ ( endpoint is not $v$), then set $c[v,d,Y,4,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,4,(+)\ell]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},4, (+)\ell]=\strue$, 
	and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,(\ssign)\srem_2]=\strue$, 
	$(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell-1\}$.
	
	\noindent {\bf Case  $\stype=5$:} If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, parent of $v$ and has one of its endpoint in $T_{\sch^v_d}$ ( endpoint is not $v$), then set $c[v,d,Y,5,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,5,(+)\ell]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},6, (+)\ell]=\strue$, and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2 \cup \{F(v)\},{\stype}_2,(+)\ell]=\strue$,  $\stype_2\in \{3,4,5\}$.
	
	\noindent {\bf Case $\stype=6$:}  If $F(v)\notin Y$, or $d=deg(v)$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, parent of $v$ and has one of its endpoint in $T_{\sch^v_{d'}}, d'>d$ (endpoint is not $v$), then set $c[v,d,Y,6,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,6,(+){\srem}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},6, (+)\ell]=\strue$, and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,(\ssign)\srem_2]=\strue$, $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell-1\}$. 
	The correctness can be argued similar to Case 5.
	
	\noindent {\bf Case  $\stype=7$:} If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, and both of its endpoint in $T_{d,i-1}$ (at least one endpoint is not $v$), then set $c[v,d,Y,7,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,7,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, $\stype_1\in \{7,8\}$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,(\ssign)\srem_2]=\strue$, $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell-1\}$. The correctness can be argued similar to Case 5.
	
	\noindent {\bf Case  $\stype=8$:} If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, and one of its endpoint in $T_{d,i-1}$ and other endpoint is in $T_{\sch^v_d}$ ($\neq v$), then set $c[v,d,Y,8,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,8,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},9, (+)\ell]=\strue$,  and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2\cup \{F(v)\},{\stype}_2,(+)\ell]=\strue$,  $\stype_2\in \{3,4,5\}$. 
	The correctness can be argued similar to Case 5.
	
	\noindent {\bf Case  $\stype=9$:} If $F(v)\notin Y$, or $d=deg(v)$ or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, and one of its endpoint in $T_{d,i-1}$ and other endpoint is in $T_{\sch^v_{d'}}$ for some $d'>d$ ($\neq v$), then set $c[v,d,Y,9,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,9,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},9, (+)\ell]=\strue$, and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,(\ssign)\srem_2]=\strue$,  $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell-1\}$. The correctness can be argued similar to Case 5.
	
	
	% \noindent {\bf Case 10} $\stype=10$ : If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, and  both of its endpoints are in $T_{\sch^v_d}$ (at least one endpoint is not equal to $v$), then set $c[v,d,Y,10,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,10,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, $\stype_1=9$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2\cup \{F(v)\},{\stype}_2,(+)\ell]=\strue$,  $\stype_2\in \{3,4,5\}$, $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell\}$. The correctness can be argued similar to Case 5.
	
	\noindent {\bf Case  $\stype=10$:} If $F(v)\notin Y$, or $d=deg(v)$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, and one of its endpoint is in $T_{\sch^v_d}$, and other endpoint is in $T_{\sch^v_{d'}}$ for some $d'>d$ ($\neq v$), then set $c[v,d,Y,10,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,10,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},11, (+)\ell]=\strue$, and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2\cup \{F(v)\},{\stype}_2,(+)\ell]=\strue$,  $\stype_2\in \{3, 4, 5\}$. The correctness can be argued similar to Case 5.
	
	\noindent {\bf Case  $\stype=11$:} If $F(v)\notin Y$, or $d=deg(v)$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, one its endpoint is in $T_{\sch^v_{d'}}$ for some $d'>d$, and other endpoint is in $T_{\sch^v_{d''}}$ for some $d''>d$ ($\neq v$), then set $c[v,d,Y,11,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,11,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds:(a1) $c[v,d-1,Y_1\cup \{F(v)\},11, (+)\ell]=\strue$,and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,(\ssign)\srem_2]=\strue$,  $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell-1\}$. The correctness can be argued similar to Case 5.
	
\end{sloppypar}

This completes the description of the (recursive) formulas for the computation of all entries of the dynamic programming table.

\noindent{\bf Correctness of recursive formulas for the computation of table entries:}

\noindent {\bf Case \stype=1:} \textbf{(1)} $\ssign=-$: Consider the case when (a1) and (a2) are true, then there exists a set of paths $\cP_1$ which set (a1) to true and there is a set of paths $\cP_2$ which set (a2) to true. We claim that $\cP=\cP_1\cup \cP_2$ is a solution to $c[v,d,Y,1,(-){\srem}]=\strue$. Observe that no path containing $v$ is in $\cP$, as $\stype=1$ in both (a1) and (a2). 
%$\stype_1,\stype_2\in \{1,2,7,8\}$. 
Since $Y=Y_1\uplus Y_2$, we have that for each $i\in Y$, we have exactly one path in $\cP\cap \cF_i$. Next, observe that there exists a vertex $u\in B$ at distance $\srem$ from $v$ in $T_{\sch^v_d}$, which is not covered by paths in $\cP_1$ and $\cP_2$. Also $(\ssign)\srem_1\in \{\sM\srem,\dots, \sP\srem-1\}$, 
$u$ is not covered by  $\cP_1$, 
as any vertex in $\cP_1$ requires at least $\srem+1$ distance to reach $u$.  Observe that every vertex at distance at least $\srem+1$ from $v$ in $T_{v,d}$ is covered by paths in $\cP$. Analogous arguments follows for the case when (b1) and (b2) are true.

\textbf{(1.1)} $\ssign=+$: Consider the case when (a1) and (a2) are true, then there exists a set of paths $\cP_1$ which set (a1) to true and there is a set of paths $\cP_2$ which set (a2) to true. We claim that $\cP=\cP_1\cup \cP_2$ is a solution to $c[v,d,Y,1,(+)\ell-1]=\strue$. 
As $\stype_2\in \{2,7,8\}$ and no path in $\cP_1$ contain $v$, 
we have that no path containing $v$ is in $\cP$. 
%Observe that no path containing $v$ is in $\cP$, as $\stype_1,\stype_2\in \{1,2,7,8\}$. 
Since $Y=Y_1\uplus Y_2$, we have that for each $i\in Y$, we have exactly one path in $\cP\cap \cF_i$. Next, observe that every vertex in $T_{\sch^v_d}$ is covered by $\cP_2$ and since  $(\ssign)\srem_1\in \{\sM\ell-2,\dots, \sP\ell-1\}$, every vertex in $T_{v,d-1}$ is covered either by $\cP_1$ or $\cP_2$. By (a2) we also satisfy $\sP\ell$, that is vertices at distance at most $\ell$ is covered by $\cP_2$. Analogous arguments follows for the case when (b1) and (b2) are true.

\textbf{(1.2)} $\ssign=+$: Consider the case when (a1) and (a2) are true, then there exists a set of paths $\cP_1$ which set (a1) to true and there is a set of paths $\cP_2$ which set (a2) to true. We claim that $\cP=\cP_1\cup \cP_2$ is a solution to $c[v,d,Y,1,(+){\srem}]=\strue$. Observe that no path containing $v$ is in $\cP$, as $\stype =1$ in (a1) and (a2). 
%$\stype_1,\stype_2\in \{1,2,7,8\}$. 
Since $Y=Y_1\uplus Y_2$, we have that for each $i\in Y$, we have exactly one path in $\cP\cap \cF_i$. Next, observe that every vertex in $T_{\sch^v_d}$ is covered by $\cP_2$ and since  $(\ssign)\srem_1\in \{\sM\srem,\dots, \sP\srem\}$, 
every vertex in $T_{v,d-1}$ is covered either by $\cP_1$ or $\cP_2$. By (a2) we also satisfy $\sP\srem$, that is vertices at distance at most $\srem$ is covered by $\cP_2$. Analogous arguments follows for the case when (b1) and (b2) are true.

\noindent {\bf Case $\stype=2$:} Suppose that (a1) and (a2) are true, then there exists a set of paths $\cP_1$ which set (a1) to true and there is a set of paths $\cP_2$ which set (a2) to true. We claim that $\cP=\cP_1\cup \cP_2 \cup \{v\}$ is a solution to $c[v,d,Y,2,(+)\ell]=\strue$. \textcolor{red}{Observe that any neighbor of $v$ cannot be there in the path $\mathcal{P}$, by observation }. Hence all the neighbors of $v$ are not in the solution. Thus $\sch^v_d$ also has $\stype=1$ in (a2). 
%Observe that no path containing $v$ is in $\cP$, as $\stype_1,\stype_2\in \{1,2,7,8\}$. 
Since $Y=Y_1\uplus Y_2\uplus \{F(v)\}$, we have that for each $i\in Y$, we have exactly one path in $\cP\cap \cF_i$. Next, observe that every vertex in $T_{\sch^v_d} \cup  T_{v,d-1}$ is covered by $\cP$ since  $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell-1\}$ and path containing $v$ is in $\cP$,  hence every vertex in $T_{v,d}$ is covered by $\cP$.

\noindent{\bf Case $\stype=5$:} Suppose that (a1) and (a2) are true, then there exists a set of paths $\cP_1$ which set (a1) to true and there is a set of paths $\cP_2$ which set (a2) to true. \textcolor{red}{}Let $P_1\in \cP_1 \subseteq \cF_{F(v)}$ and let $P_2\in \cP_1 \subseteq \cF_{F(v)}$. Observe that $\cP^*_1=(\cP_1\setminus \{P_1\})\cup \{P_2\}$ also sets (a1) to true. We claim that $\cP=\cP^*_1\cup \cP_2$ is also a solution to $c[v,d,Y,5,(+)\ell]=\strue$.  since $Y=Y_1\uplus Y_2\uplus \{F(v)\}$, and $\stype_1=6$ and $\stype_2\in \{3,4,5\}$, and exactly one path containing $v$ is in $\cP$,  we have that for each $i\in Y$, we have exactly one path in $\cP\cap \cF_i$. Next, observe that every vertex in $T_{\sch^v_d} \cup T_{v,d-1}$ is covered by $\cP$, hence every vertex in $T_{v,d}$ is covered by $\cP$.

Correctness of remaining cases can be argued similar to above cases.

\noindent{\bf Running time:} The correctness of the algorithm follows from the correctness of the (recursive) formulas, and the fact $(T,B,\ell,\cF=\{\cF_1,\cF_2,\dots, \cF_t\})$ is a yes instance of \amesp if and only if there exists an entry $c[r,deg(r),Y,\stype^*,\sP\srem^*]$, $\stype^*\in \{1,2,7,8\}$ and  $\srem^* \in [0,\ell]$, which is set to $\strue$. Next, we analyse the running time of our algorithm. Recall that $|\cF|\leq t$. Observe that each of our table entry can be computed in time $\OO(\ell 2^t)$. The number of entries are bounded by $\OO(\ell 2^t n^{\OO(1)})$. Therefore, the running time of our algorithm is bounded by $\OO(\ell 2^{\OO(t)} n^{\OO(1)})$. This completes the proof of \cref{thm:annotated}.



%{\em Correctness}: Suppose that (a1) and (a2) are true, then there exists a set of paths $\cP_1$ which set (a1) to true and there is a set of paths $\cP_2$ which set (a2) to true. Let $P_1\in \cP_1 \subseteq \cF_F(v)$ and let $P_2\in \cP_1 \subseteq \cF_F(v)$. Observe that $\cP^*_1=(\cP_1\setminus \{P_1\})\cup \{P_2\}$ also sets (a1) to true. We claim that $\cP=\cP^*_1\cup \cP_2$ is also a solution to $c[v,d,Y,5,(+)\ell]=\strue$.  since $Y=Y_1\uplus Y_2\uplus \{F(v)\}$, and $\stype_1=6$ and $\stype_2\in \{3,4,5\}$, and exactly one path containing $v$ is in $\cP$,  we have that for each $i\in Y$, we have exactly one path in $\cP\cap \cF_i$. Next, observe that every vertex in $T_{\sch^v_d} \cup T_{v,d-1}$ is covered by $\cP$, hence every vertex in $T_{v,d}$ is covered by $\cP$.

%\noindent {\bf Case 6} $\stype=6$ : If $F(v)\notin Y$, or $d=deg(v)$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, parent of $v$ and has one of its endpoint in $T_{\sch^v_{d'}}, d'>d$ (endpoint is not $v$), then set $c[v,d,Y,6,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,6,(+){\srem}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, and (a2) $c[\sch^v_i,deg(\sch^v_i),Y_2,{\stype}_2,(+)\ell]=\strue$, where $\stype_1,\stype_2=6$. The correctness can be argued similar to Case 5.
%
%\noindent {\bf Case 7} $\stype=7$ : If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, and both of its endpoint in $T_{d,i-1}$ (at least one endpoint is not $v$), then set $c[v,d,Y,7,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,7,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, $\stype_1\in \{7,8,9\}$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,{\stype}_2,(\ssign)\srem_2]=\strue$,  $\stype_2 \in \{1,2,7,8\}$, $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell\}$. The correctness can be argued similar to Case 5.
%
%\noindent {\bf Case 8} $\stype=8$ : If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, and one of its endpoint in $T_{d,i-1}$ and other endpoint is in $T_{\sch^v_d}$ ($\neq v$), then set $c[v,d,Y,8,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,8,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, $\stype_1=9$ and (a2) $c[\sch^v_i,deg(\sch^v_i),Y_2\cup \{F(v)\},{\stype}_2,(+)\ell]=\strue$,  $\stype_2\in \{3,4,5\}$, $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell\}$. The correctness can be argued similar to Case 5.
%
%\noindent {\bf Case 9} $\stype=9$ : If $F(v)\notin Y$, or $d=deg(v)$ or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, and one of its endpoint in $T_{d,i-1}$ and other endpoint is in $T_{\sch^v_{d'}}$ for some $d'>d$ ($\neq v$), then set $c[v,d,Y,9,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,9,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, $\stype_1=9$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,{\stype}_2,(+)\ell]=\strue$,  $\stype_2\in \{1,2,7,8\}$, $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell\}$. The correctness can be argued similar to Case 5.
%
%
%% \noindent {\bf Case 10} $\stype=10$ : If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, and  both of its endpoints are in $T_{\sch^v_d}$ (at least one endpoint is not equal to $v$), then set $c[v,d,Y,10,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,10,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, $\stype_1=9$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2\cup \{F(v)\},{\stype}_2,(+)\ell]=\strue$,  $\stype_2\in \{3,4,5\}$, $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell\}$. The correctness can be argued similar to Case 5.
% 
% \noindent {\bf Case 10} $\stype=10$ : If $F(v)\notin Y$, or $d=deg(v)$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, and one of its endpoint is in $T_{\sch^v_d}$, and other endpoint is in $T_{\sch^v_{d'}}$ for some $d'>d$ ($\neq v$), then set $c[v,d,Y,10,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,10,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, $\stype_1=12$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2\cup \{F(v)\},{\stype}_2,(+)\ell]=\strue$,  $\stype_2=11$. The correctness can be argued similar to Case 5.
% 
% \noindent {\bf Case 11} $\stype=11$ : If $F(v)\notin Y$, or $d=deg(v)$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, one its endpoint is in $T_{\sch^v_{d'}}$ for some $d'>d$, and other endpoint is in $T_{\sch^v_{d''}}$ for some $d''>d$ ($\neq v$), then set $c[v,d,Y,11,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,11,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds:(a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, $\stype_1=12$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,{\stype}_2,(+)\ell]=\strue$,  $\stype_2\in \{1,2,7,8\}$, $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell\}$. The correctness can be argued similar to Case 5.
%
\end{sloppypar}
%
%Due to space constraints we add description of the formulas for the remaining cases and correctness for algorithm and running time analysis in \cref{sec:annotatedapp}. 
%The correctness of the algorithm follows from the correctness of the (recursive) formulas, and the fact $(T,B,\ell,\cF=\{\cF_1,\cF_2,\dots, \cF_t\})$ is a yes instance of \amesp if and only there exists an entry $c[r,deg(r),\stype^*,\sP\srem^*]$, $\stype^*\in \{1,2,7,8\}$ and  $\srem^* \in [0,\ell]$, which is set to $\strue$. Next, we analyse the running time of our algorithm. Recall that $|\cF|\leq t$. Observe that for each of our table entry can be computed in time $\OO(\ell 2^t)$ time. The number of entries are bounded by $\OO(\ell 2^t n^{\OO(1)})$. Therefore the running time of our algorithm is bounded by $\OO(\ell 2^t n^{\OO(1)})$. This completes the proof of \cref{lem:annotated}.

==> fvsdp.tex <==
\subsection{Algorithm for \annotatedmesp \textcolor{red}{Previous version}}\label{sec:annotated1}

In this section, we design a dynamic programming based FPT algorithm for \amesp problem.  In particular we prove \cref{thm:annotated}. Consider an instance $(T,B,\ell,\cF =\{\cF_1,\cF_2,\dots \cF_t\})$ of \amesp problem. Recall that $T$ is a tree, $B\subseteq V(T)$, $\ell\in \mathbb{N}$, and $\cF$ satisfy the following: (1) Each $\cF_i$, $i\in [t]$ is a set of paths in $T$, and (2) $V(\cF_i)\cap V(\cF_j)=\emptyset$, for all $i,j\in [t], i\neq j$. The aim is to find a set $\cal P$ of $t$ paths such that for each $\cF_i$, $i\in [t]$, $\mathcal{P}\cap \cF_i=1$ and for every vertex $v\in B$, there exists a path $P\in {\cal P}$ and a vertex $u\in V(P)$, such that $d_T(u,v)\leq \ell$. 



% (3) If there exists two paths $P_1,P_2\in \cF_i$, $i\in [t]$, with endpoints $u_1,v_1$ and $u_2,v_2$, respectively, such that $V(P_1)\cap V(P_2)\neq \emptyset$, then there exists a vertex $v\in V(P_1)\cap V(P_2)$ such that $P_1$ and $P_2$ are paths that passes through $v$ and one of the following holds: 
%(i) Their endpoints are distinct, i.e., $u_1\neq u_2, u_1\neq v_2, v_1\neq u_2, v_1\neq v_2$ and 
%
%$V(P_1)\cap V(P_2)= \{v\}$.
%
%(ii) One of the endpoint is equal, for example $u_1=u_2$ and $v_1\neq v_2$ (other cases are analogous), in this case let $P'$ be the $v$ to $u_1$ subpath in $T$, then $V(P_1)\cap V(P_2)= V(P')$. 





%We design a dynamic programming algorithm. Intuition..



First we give the description of our algorithm. The algorithm starts by arbitrarily rooting tree $T$ at a root $r\in V(T)$. From now onwards, we assume that $T$ is rooted at $r$. In the following, we state some notations, which will be used in the algorithm. For a vertex $v\in V(T)$, we denote the number of children of $v$ in $T$ by $deg(v)$. By $T_v$, we denote the subtree of $T$ rooted at $v$. For a vertex $v\in T$, and  $0 \leq i\leq deg(v)$, we define $T_{v,i}$ as the subtree of $T$ containing vertex $v$ and subtrees rooted at its first $i$ children (in order of index). Recall that every vertex $v\in V(T)$ can be contained in at most one $\cF_i$, $i\in[t]$. For each vertex $v\in V(T)$, we assign a value $F(v)\in [0,t]$ to $v$ as follows: $F(v)=i$, if $v\in V(\cF_i)$, $0$ otherwise (when no path in any $\cF_i, i\in [t]$ contain $v$). By $\sch^v_i$, we denote $i$th child of $v$. Recall that   a path $P$ {\em covers} a vertex $v$ if there exists a vertex $u\in V(P)$ such that $d_{G}(v,u)\leq \ell$. For a vertex $v\in V(T)$, dynamic programming algorithm considers subproblems for each child of $v$. We process its children from left to right (in index ordering) and at $i$th child, we consider subtree $T_{v,i}$. Before we define an entry in the table, we give the definition of the variables used for an entry. 
  
 Consider $v\in V(T)$ and $i\in [deg(v)]$. To compute partial solution at subtree $T_{v,i}$, we have to distinguish whether $v$ is contained in a path in the solution. If it is contained in a path in the solution, then we also guess where  the endpoints of the path are. For this purpose, we define a variable $\stype$ which can take a value from the set $\{1, 2, \dots, 11\}$, where each value represents a different case which are as follows: $\bf (1)$ Paths containing $v$ should not be in the solution. 
 $\bf (2)$ The vertex $v$ itself is a path that is contained in solution. For the remaining cases we have that a path containing $v$ is in the solution with the following added conditions: For $\stype\in \{3,4,5,6\}$, cases {\bf (3),(4),(5)} and {\bf (6)} we have condition that path also contains parent of $v$: with the following added conditions:
 $\bf (3)$ One of its endpoint is $v$ itself. 
 $\bf (4)$ One of its endpoint is in $T_{v,i-1}$ ($\neq v$). 
  $\bf (5)$ One of its endpoint is in $T_{\sch^v_i}$ ($\neq v$). 
  $\bf (6)$ One of its endpoint is in $T_{\sch^v_j}$ for some $j>i$ ($\neq v$).
  $\bf (7)$ Both of its endpoints are in $T_{v,i-1}$ (at least one endpoint is not equal to $v$).
  $\bf (8)$ One of its endpoint is in $T_{v,i-1}$, and other endpoint is in $T_{\sch^v_i}$ ($\neq v$). 
  $\bf (9)$ One of its endpoint is in $T_{v,i-1}$, and other endpoint is in $T_{\sch^v_j}$ for some $j>i$ ($\neq v$). 
%\item $\bf 10$ represents that a path containing $v$ is in the solution and both of its endpoints are in $T_{\sch^v_i}$ (at least one endpoint is not equal to $v$).
  $\bf (10)$ One of its endpoint is in $T_{\sch^v_i}$, and other endpoint is in $T_{\sch^v_j}$ for some $j>i$ ($\neq v$). 
  $\bf (11)$ One its endpoint is in $T_{\sch^v_j}$ for some $j>i$, and other endpoint is in $T_{\sch^v_{j'}}$ for some $j'>i$ ($\neq v$). 

%\end{itemize}


\begin{sloppypar}
We have a variable $(\ssign)\srem$. Here $\ssign$ represents sign of $\srem$, which can be either $+$ or $-$, and $(\ssign)\srem$ can take a value from the set $\{\sM\ell-1,\dots, \sM1, \sM0,\sP0,\sP1,\dots, \sP \ell\}$. The ``$-$'' sign represents that there are uncovered vertices in $V(T_{v,i})\cap B$ which needs to be covered in future, and ``$+$'' sign represents that all the vertices in $V(T_{v,i})\cap B$ are covered and partial solution may cover more vertices outside $T_{v,i}$. The value $\sM\srem$ represents maximum distance of a vertex $u\in B$ from $v$ in subtree $T_{v,i}$ such that $u$ is not covered by the partial solution is $\srem$. It means that vertices up to distance $\srem$ from $v$ in $V(T_{v,i})\cap B$ needs to be covered by some paths in future. We consider values only till $\ell-1$ distance, as it is a trivial observation that any vertex at distance at least $\ell$ from $v$ in $T_{v,i}$ cannot be covered by any path that is not in $T_{v,i}$. The value $\sP\srem$ represents the minimum value such that there exists a vertex $u\in B$ in subtree $T_{v,i}$ such that distance from $u$ to $v$ is $\ell-\srem$ and $u$ is contained in a path in the solution. It means that vertices in $B$ which are at distance at most $\srem$ from $v$ (at most $\ell$ from $u$) in $T$ can be covered by a path containing $u$ in the solution. In the following definition, we state the entries in our dynamic programming routine.
 
%We have a variable $\srem$, it can take a value from set $[-1,\ell-1]$ which represents maximum distance of a vertex $u$ from $v$ in subtree $T_{v,i}$ such that $u$ is not covered by the partial solution. It means that vertices up to distance $\srem$ from $v$ in $T_{v,i}$ needs to be covered by some paths in future. $-1$ represents that all the vertices in $T_{v,i}$ are covered. We consider only till $\ell-1$ distance, as it is a trivial observation that any vertex at distance at least $\ell$ from $v$ in $T_{v,i}$ cannot be covered by any path that is not in $T_{v,i}$.
%
%We have a variable $\sf ext$, it can take a value from the set $[0,\ell]$, it represents that (1) every vertex in $T_{v,i}$ is covered and (2) $\sf ext$ is the minimum value such that there exists a vertex $u$ in subtree $T_{v,i}$ such that distance from $u$ to $v$ is $\ell-\sext$ and $u$ contained in a path in the solution. It means that vertices at distance at most $\sf ext$ from $v$ ( at most $\ell$ from $u$) should be covered by a path contaning $u$ in the solution.


%We have a variable $\srem$, it can take a value from set $[-1,\ell-1]$ which represents distance from $v$ to a vertex $u$ in subtree $T_{v,i}$ such that $v$ is not covered by the partial solution. It means that vertices up to distance $\srem$ from $v$ in $T_{v,i}$ needs to be covered by some paths in future. $-1$ represents that all the vertices in $T_{v,i}$ are covered. We consider only till $\ell-1$ distance, as it is a trivial observation that any vertex at distance at least $\ell$ from $v$ in $T_{v,i}$ cannot be covered by any path that is not in $T_{v,i}$.
%
%We have a variable $\sf ext$, it can take a value from the set $[\ell]$, which represents $\ell$ minus minimum distance from $v$ to a vertex $u$ in subtree $T_{v,i}$ such that $u$ contained in a path in the solution. It means that vertices at distance at most $\sf ext$ from $v$ ( at most $\ell$ from $u$) should be covered by a path contaning $u$ in the solution.

% In the following definition, we state the entries in our dynamic programming routine.
% 
% \begin{definition} For each $v\in V(T)$, $d\in deg(v)$, $Y\subseteq [t]$,$\stype\in [12]$, ${\sf ext}\in [\ell], {\srem}\in [-1,\ell-1]$ we store an entry $c[v,d,Y,{\stype}, {\sf ext}, {\srem}]$ in our table which stores $\strue$ if and only if the following holds:

\begin{definition} \label{def:dp}
For each $v\in V(T)$, $d\in deg(v)$, $Y\subseteq [t]$,$\stype\in \{1, 2,\dots, 11\}, (\ssign)\srem \in\{\sM\ell-1,\dots, \sM1, \sM0,\sP0,\sP1,\dots, \sP \ell\}$ we store an entry $c[v,d,Y,{\stype},(\ssign) {\srem}]$ in our table which stores $\strue$ if and only if the following holds, otherwise $c[v,d,Y,{\stype}, {\srem}]$ stores $\sfalse$:
 {\bf (1)} There exists a set $\cP_{v,d}$ of $|Y|$ paths such that for each $j\in Y$, $|\cP_{v,d}\cap \cF_j|=1$, if $F(v)\in Y$, then path in $\cP_{v,d}\cap \cF_{F(v)}$ should satisfy definition of $\stype$, and all paths in $\cP_{v,d}$ except maybe path containing $v$ should be contained in the subtree $T_{v,d}$. {\bf (2)} If $\ssign$ is $-$, then there exists a vertex $u\in B$ at distance $\srem$  from $v$ in $T_{v,d}$ which is not covered by any paths in $\cP_{v,d}$ but can be covered in future (is not at distance greater than $\ell$ from $v$). For every vertex $u\in B$ at distance at least ${\srem} +1$ from $v$ in subtree $T_{v,d}$ there exists a path in $\cP_{v,d}$ which covers $u$. {\bf (3)} If $\ssign$ is $+$, then for every vertex $u\in B$ which is either in $T_{v,d}$, or not in $T_{v,d}$ and at a distance at most ${\srem}$ from $v$ there exists a path in $\cP_{v,d}$ which covers $u$.  
 \end{definition}

\begin{comment}
\textcolor{red}{
\begin{observation}\label{obs:new-dp1}
Let $v\in V(T)$ and $w$ be a child of $v$ and 
the solution set $\mathcal{P}_{r, deg(r)}$ be the set of paths at root $r$, satisfying the rules of Definition \ref{def:dp}. If $v$ and $w$ belong to some paths $P$ in $\mathcal{P}_{r, deg(r)}$, then 
$F(v)=F(w)$. 
%$\mathcal{P}_{v,d}$ denote the set of paths in the solution satisfying Definition \ref{def:dp}. 
%If there exists a vertex $w\in N(v)$ such that $\mathcal{F}_{(F(w))}\in \mathcal{P}$, then $F(w)=F(v)$. 
%$f(w)\neq f(v)$. 
\end{observation}
\begin{proof}
%Suppose Since $v\in S$, we have that $F(v)\in [t]$. 
There are two cases depending on whether $v$ and $w$ belong to the same path or different paths in the solution. Let they belong to different paths. There exists a shortest path between endpoints (in $M$) 
in the path containing $v$ and the endpoints (in $M$) in the path of $w$. These are  not valid paths to be considered in the instance. The other case is that there is path containing $v$ and $w$ in the solution. Hence $F(v)=F(w)$. 
%Suppose $F(v)\neq F(w)$. That is there exists paths $P_v$ and $P_w$ passing through $v$ (and not $w$) and $w$ (and not $v$). 
%Let $P_v$ be the path in $\mathcal{}$the Then there exists a shortest path passing through the vertices of $M$ passing through $v$, $w$ and then to the vertices in $M$. 
\end{proof}}

\end{comment}



Observe that $(T,B,\ell,\cF=\{\cF_1,\cF_2,\dots,  \cF_t\})$ is a yes instance of \amesp if and only if there exists an entry $c[r,deg(r),Y, \stype^*,\sP\srem^*]$, $\stype^*\in \{1,2,7,8\}$ and  $\srem^* \in [0,\ell]$, which is set to $\strue$. Next, we give (recursive) formulas for the computation of entries in our dynamic programming table. Their correctness can be found in \cref{sec:annotatedapp}~. 
Consider $v\in V(T),d\in deg(v),Y\subseteq [t],\stype\in [11],  (\ssign)\srem \in \{\sM\ell-1,\dots, \sM1, \sM0,\sP0,\sP1,\dots, \sP \ell\}$, 
we compute the entry $c[v,d,Y,{\stype}, (\ssign){\srem}]$ based on the following cases: 

\noindent{\bf $v$ is a leaf vertex:} 
%$v$ is a leaf vertex. 
Set $c[v,d,Y,{\stype}, (\ssign){\srem}]=\strue$, if one of the following holds: (i) $\stype=1, (\ssign)\srem=\sM 0$, $Y=\emptyset$, or (ii) $\stype\in \{2,3\} , (\ssign)\srem=\sP\ell$, $F(v)=Y$. Otherwise set the entry to $\sfalse$. Note that here $d=0$. 
Correctness follows trivially from the definition of entry. 

\noindent{\bf $v$ is a non-leaf vertex:} 
%$v$ is not a leaf vertex. 
We consider following cases depending on $\stype$ variable. 

\noindent {\bf Case 1} $\stype=1$ : We further consider following cases.
(1) If $\ssign=-$, then set $c[v,d,Y,1,(-){\srem}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y$ such that one of the following holds: 

\noindent
%(a1) $c[v,d-1,Y_1,{\stype}_1, (\ssign){\srem}_1]=\strue$,  $\stype_1\in \{1,2,7,8\}$, $(\ssign)\srem_1\in \{\sM\srem-1,\dots, \sP\srem\}$ and
% (a2) $c[\sch^v_d,deg(\sch^v_i),Y_2,\stype_2,\sM\srem-1]=\strue$, $\stype_2\in \{1,2,7,8\}$, or 
 (a1) $c[v,d-1,Y_1,1, (\ssign){\srem}_1]=\strue$,  $(\ssign)\srem_1\in \{\sM\srem,\dots, \sP\srem\}$ and
 (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,\sM\srem-1]=\strue$, or,  
 (b1) $c[v,d-1,Y_1,1, \sM{\srem}]=\strue$, and
 (b2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,(\ssign)\srem_2]=\strue$, $(\ssign)\srem_2\in \{\sM\srem-1,\dots, \sP\srem\}$. 
 %where 
 %$\srem\neq \ell-1$,  or, 
 % (c1) $c[v,d-1,Y_1,1, \sM{\ell-1}]=\strue$, and
 %(c2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,(\ssign)\srem_2]=\strue$, $(\ssign)\srem_2\in \{\sM\srem-1,\dots, \sP\ell -\srem+2\}$. 


%{\em Correctness}: Consider the case when (a1) and (a2) are true, then there exists a set of paths $\cP_1$ which set (a1) to true and there is a set of paths $\cP_2$ which set (a2) to true. We claim that $\cP=\cP_1\cup \cP_2$ is a solution to $c[v,d,Y,1,(-){\srem}]=\strue$. Observe that no path containing $v$ is in $\cP$, as $\stype_1,\stype_2\in \{1,2,7,8\}$. since $Y=Y_1\uplus Y_2$, we have that for each $i\in Y$, we have exactly one path in $\cP\cap \cF_i$. Next, observe that there exists a vertex $u\in B$ at distance $\srem$ from $v$ in $T_{\sch^v_d}$, which is not covered by paths in $\cP_1$. Also $(\ssign)\srem_1\in \{\sM\srem-1,\dots, \sP\srem\}$, it is not covered by  $\cP_2$, as any vertex in $\cP_2$ requires at least $\srem+1$ distance to reach $u$. Observe that every vertex at distance at least $\srem+1$ from $v$ in $T_{v,d}$ is covered by paths in $\cP$. Analogous arguments follows for the case when (b1) and (b2) are true.




(2.1) If $\ssign=+$, then set $c[v,d,Y,1,(+)\ell -1]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y$ such that one of the following holds: (a1) $c[v,d-1,Y_1,1, (\ssign)\srem_1]=\strue$,   $(\ssign)\srem_1\in \{\sM\ell-2,\dots, \sP\ell-1\}$ and
 (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,\stype_2,\sP\ell]=\strue$, $\stype_2\in \{2,7,8\}$, or, 
  (b1) $c[v,d-1,Y_1,1, \sP\ell-1]=\strue$, 
  and
 (b2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,(\ssign)\srem_2]=\strue$, $(\ssign)\srem_2\in \{\sM\ell-2,\dots, \sP\ell-1\}$. 


 
 
 
(2.2) If $\ssign=+$ and $\srem<\ell-1$, then set $c[v,d,Y,1,(+){\srem}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y$ such that one of the following holds: (a1) $c[v,d-1,Y_1,1, (\ssign){\srem}_1]=\strue$,  $(\ssign)\srem_1\in \{\sM\srem,\dots, \sP\srem\}$ and
 (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,\sP\srem+1]=\strue$,  or
  (b1) $c[v,d-1,Y_1,1, \sP{\srem}]=\strue$,  and
 (b2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,(\ssign)\srem_2]=\strue$,  $(\ssign)\srem_2\in \{\sM\srem,\dots, \sP\srem+1\}$.



%\bscomment{**}
%{\em Correctness}: Consider the case when (a1) and (a2) are true, then there exists a set of paths $\cP_1$ which set (a1) to true and there is a set of paths $\cP_2$ which set (a2) to true. We claim that $\cP=\cP_1\cup \cP_2$ is a solution to $c[v,d,Y,1,(+){\srem}]=\strue$. Observe that no path containing $v$ is in $\cP$, as $\stype_1,\stype_2\in \{1,2,7,8\}$. since $Y=Y_1\uplus Y_2$, we have that for each $i\in Y$, we have exactly one path in $\cP\cap \cF_i$. Next, observe that every vertex in $T_{\sch^v_d}$ is covered by $\cP_2$ and since  $(\ssign)\srem_1\in \{\sM\srem,\dots, \sP\srem+1\}$, every vertex in $T_{v,d-1}$ is covered either by $\cP_1$ or $\cP_2$. By (a2) we also satisfy $\sP\srem$, that is vertices at distance at most $\srem$ is covered by $\cP_2$. Analogous arguments follows for the case when (b1) and (b2) are true.

\noindent {\bf Case 2} $\stype=2$ : If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or $v$ is not a path in $\cF_{F(v)}$, then set $c[v,d,Y,2,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,2,(+)\ell]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1,2, \sP\ell]=\strue$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,1,(\ssign)\srem_2]=\strue$,  $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell-1\}$.


%{\em Correctness}: Suppose that (a1) and (a2) are true, then there exists a set of paths $\cP_1$ which set (a1) to true and there is a set of paths $\cP_2$ which set (a2) to true. We claim that $\cP=\cP_1\cup \cP_2 \cup \{v\}$ is a solution to $c[v,d,Y,2,(+)\ell]=\strue$. Observe that no path containing $v$ is in $\cP$, as $\stype_1,\stype_2\in \{1,2,7,8\}$. since $Y=Y_1\uplus Y_2\uplus \{F(v)\}$, we have that for each $i\in Y$, we have exactly one path in $\cP\cap \cF_i$. Next, observe that every vertex in $T_{\sch^v_d} \cup  T_{v,d-1}$ is covered by $\cP$ since  $(\ssign)\srem_1\in \{\sM\srem,\dots, \sP\srem+1\}$ and path containing $v$ is in $\cP$,  hence every vertex in $T_{v,d}$ is covered by $\cP$.

%\noindent {\bf Case 3} $\stype=3$ : If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, parent of $v$ and has one of its endpoint as $v$, then set $c[v,d,Y,3,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,3,(+)\ell]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},3, (+)\ell]=\strue$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,{\stype}_2,(\ssign)\srem_2]=\strue$,  $\stype_2\in \{1,2,7,8\}$, $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell\}$.
%% The correctness can be argued similar to Case 2.
%
%\noindent {\bf Case 4} $\stype=4$ : If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, parent of $v$ and has one of its endpoint in $T_{v,d-1}$ ( endpoint is not $v$), then set $c[v,d,Y,4,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,4,(+)\ell]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, $\stype\in \{3,4\}$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,{\stype}_2,(\ssign)\srem_2]=\strue$,  $\stype_2\in \{1,2,7,8\}$, $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell\}$.
% The correctness can be argued similar to Case 2.

\noindent {\bf Case 5} $\stype=5$ : If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, parent of $v$ and has one of its endpoint in $T_{\sch^v_d}$ ( endpoint is not $v$), then set $c[v,d,Y,5,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,5,(+)\ell]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},6, (+)\ell]=\strue$, and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2 \cup \{F(v)\},{\stype}_2,(+)\ell]=\strue$,  $\stype_2\in \{3,4,5\}$. 


%{\em Correctness}: Suppose that (a1) and (a2) are true, then there exists a set of paths $\cP_1$ which set (a1) to true and there is a set of paths $\cP_2$ which set (a2) to true. Let $P_1\in \cP_1 \subseteq \cF_F(v)$ and let $P_2\in \cP_1 \subseteq \cF_F(v)$. Observe that $\cP^*_1=(\cP_1\setminus \{P_1\})\cup \{P_2\}$ also sets (a1) to true. We claim that $\cP=\cP^*_1\cup \cP_2$ is also a solution to $c[v,d,Y,5,(+)\ell]=\strue$.  since $Y=Y_1\uplus Y_2\uplus \{F(v)\}$, and $\stype_1=6$ and $\stype_2\in \{3,4,5\}$, and exactly one path containing $v$ is in $\cP$,  we have that for each $i\in Y$, we have exactly one path in $\cP\cap \cF_i$. Next, observe that every vertex in $T_{\sch^v_d} \cup T_{v,d-1}$ is covered by $\cP$, hence every vertex in $T_{v,d}$ is covered by $\cP$.

%\noindent {\bf Case 6} $\stype=6$ : If $F(v)\notin Y$, or $d=deg(v)$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, parent of $v$ and has one of its endpoint in $T_{\sch^v_{d'}}, d'>d$ (endpoint is not $v$), then set $c[v,d,Y,6,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,6,(+){\srem}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, and (a2) $c[\sch^v_i,deg(\sch^v_i),Y_2,{\stype}_2,(+)\ell]=\strue$, where $\stype_1,\stype_2=6$. The correctness can be argued similar to Case 5.
%
%\noindent {\bf Case 7} $\stype=7$ : If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, and both of its endpoint in $T_{d,i-1}$ (at least one endpoint is not $v$), then set $c[v,d,Y,7,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,7,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, $\stype_1\in \{7,8,9\}$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,{\stype}_2,(\ssign)\srem_2]=\strue$,  $\stype_2 \in \{1,2,7,8\}$, $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell\}$. The correctness can be argued similar to Case 5.
%
%\noindent {\bf Case 8} $\stype=8$ : If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, and one of its endpoint in $T_{d,i-1}$ and other endpoint is in $T_{\sch^v_d}$ ($\neq v$), then set $c[v,d,Y,8,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,8,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, $\stype_1=9$ and (a2) $c[\sch^v_i,deg(\sch^v_i),Y_2\cup \{F(v)\},{\stype}_2,(+)\ell]=\strue$,  $\stype_2\in \{3,4,5\}$, $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell\}$. The correctness can be argued similar to Case 5.
%
%\noindent {\bf Case 9} $\stype=9$ : If $F(v)\notin Y$, or $d=deg(v)$ or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, and one of its endpoint in $T_{d,i-1}$ and other endpoint is in $T_{\sch^v_{d'}}$ for some $d'>d$ ($\neq v$), then set $c[v,d,Y,9,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,9,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, $\stype_1=9$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,{\stype}_2,(+)\ell]=\strue$,  $\stype_2\in \{1,2,7,8\}$, $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell\}$. The correctness can be argued similar to Case 5.
%
%
%% \noindent {\bf Case 10} $\stype=10$ : If $F(v)\notin Y$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, and  both of its endpoints are in $T_{\sch^v_d}$ (at least one endpoint is not equal to $v$), then set $c[v,d,Y,10,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,10,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, $\stype_1=9$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2\cup \{F(v)\},{\stype}_2,(+)\ell]=\strue$,  $\stype_2\in \{3,4,5\}$, $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell\}$. The correctness can be argued similar to Case 5.
% 
% \noindent {\bf Case 10} $\stype=10$ : If $F(v)\notin Y$, or $d=deg(v)$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, and one of its endpoint is in $T_{\sch^v_d}$, and other endpoint is in $T_{\sch^v_{d'}}$ for some $d'>d$ ($\neq v$), then set $c[v,d,Y,10,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,10,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds: (a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, $\stype_1=12$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2\cup \{F(v)\},{\stype}_2,(+)\ell]=\strue$,  $\stype_2=11$. The correctness can be argued similar to Case 5.
% 
% \noindent {\bf Case 11} $\stype=11$ : If $F(v)\notin Y$, or $d=deg(v)$, or $\ssign=\sM$, or $\srem\neq \ell$, or there is no path in $\cF_{F(v)}$ containing $v$, one its endpoint is in $T_{\sch^v_{d'}}$ for some $d'>d$, and other endpoint is in $T_{\sch^v_{d''}}$ for some $d''>d$ ($\neq v$), then set $c[v,d,Y,11,(\ssign){\srem}]=\sfalse$. Correctness follows trivially. Otherwise we set $c[v,d,Y,11,(+){\ell}]=\strue$ if there exists a partition $Y_1\uplus Y_2$ of $Y\setminus \{F(v)\}$ such that the following holds:(a1) $c[v,d-1,Y_1\cup \{F(v)\},\stype_1, (+)\ell]=\strue$, $\stype_1=12$ and (a2) $c[\sch^v_d,deg(\sch^v_d),Y_2,{\stype}_2,(+)\ell]=\strue$,  $\stype_2\in \{1,2,7,8\}$, $(\ssign)\srem_2\in \{\sM\ell-1,\dots, \sP\ell\}$. The correctness can be argued similar to Case 5.
%
\end{sloppypar}
%
Due to space constraints we add description of the formulas for the remaining cases and correctness for algorithm and running time analysis in \cref{sec:annotatedapp}. 
%The correctness of the algorithm follows from the correctness of the (recursive) formulas, and the fact $(T,B,\ell,\cF=\{\cF_1,\cF_2,\dots, \cF_t\})$ is a yes instance of \amesp if and only there exists an entry $c[r,deg(r),\stype^*,\sP\srem^*]$, $\stype^*\in \{1,2,7,8\}$ and  $\srem^* \in [0,\ell]$, which is set to $\strue$. Next, we analyse the running time of our algorithm. Recall that $|\cF|\leq t$. Observe that for each of our table entry can be computed in time $\OO(\ell 2^t)$ time. The number of entries are bounded by $\OO(\ell 2^t n^{\OO(1)})$. Therefore the running time of our algorithm is bounded by $\OO(\ell 2^t n^{\OO(1)})$. This completes the proof of \cref{lem:annotated}.
